Deep Reinforcement Learning for Modelling Protein Complexes

AlphaFold can be used for both single-chain and multi-chain protein structure prediction, while the latter becomes extremely challenging as the number of chains increases. In this work, by taking each chain as a node and assembly actions as edges, we show that an acyclic undirected connected graph can be used to predict the structure of multi-chain protein complexes (a.k.a., protein complex modelling, PCM). However, there are still two challenges: 1) The huge combinatorial optimization space of $N^{N-2}$ ($N$ is the number of chains) for the PCM problem can easily lead to high computational cost. 2) The scales of protein complexes exhibit distribution shift due to variance in chain numbers, which calls for the generalization in modelling complexes of various scales. To address these challenges, we propose GAPN, a Generative Adversarial Policy Network powered by domain-specific rewards and adversarial loss through policy gradient for automatic PCM prediction. Specifically, GAPN learns to efficiently search through the immense assembly space and optimize the direct docking reward through policy gradient. Importantly, we design an adversarial reward function to enhance the receptive field of our model. In this way, GAPN will simultaneously focus on a specific batch of complexes and the global assembly rules learned from complexes with varied chain numbers. Empirically, we have achieved both significant accuracy (measured by RMSD and TM-Score) and efficiency improvements compared to leading PCM softwares.

==> table/table-1.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[h]
\setlength{\tabcolsep}{2pt}
\renewcommand\arraystretch{1.5}
\centering
\resizebox{0.95\textwidth}{!}{%
\begin{tabular}{@{}lccccccccc@{}}
\toprule
             & \multicolumn{3}{c|}{\textbf{\texttt{\scalebox{1.2}{GT Dimer}}}} & \multicolumn{3}{c|}{\textbf{\texttt{\scalebox{1.2}{AF-MM Dimer}}}} & \multicolumn{3}{c}{\textbf{\texttt{\scalebox{1.2}{ESMFold Dimer}}}} \\ \cmidrule(l){2-10} 
\multirow{-2}{*}{\textbf{\scalebox{1.3}{Methods}}} &
  RMSD ($\uparrow$) &
  TM-Score ($\uparrow$) &
  \multicolumn{1}{c|}{DockQ ($\uparrow$)} &
  RMSD ($\uparrow$) &
  TM-Score ($\uparrow$) &
  \multicolumn{1}{c|}{DockQ ($\uparrow$)} &
  RMSD ($\uparrow$) &
  TM-Score ($\uparrow$) &
  DockQ ($\uparrow$) \\ \midrule
\scalebox{1.2}{Multi-Zerd}   &   &   & \multicolumn{1}{c|}{} &    &    & \multicolumn{1}{c|}{}  &           &           &           \\
\scalebox{1.2}{RL-MLZerD} &   &   & \multicolumn{1}{c|}{} &    &    & \multicolumn{1}{c|}{}  &           &           &           \\
\scalebox{1.2}{AF-Multimer}  &   &   & \multicolumn{1}{c|}{} &    &    & \multicolumn{1}{c|}{}  &           &           &           \\
\scalebox{1.2}{ESMFold}      &   &   & \multicolumn{1}{c|}{} &    &    & \multicolumn{1}{c|}{}  &           &           &           \\
\scalebox{1.2}{MoLPC}        &   &   & \multicolumn{1}{c|}{} &    &    & \multicolumn{1}{c|}{}  &           &           &           \\
\scalebox{1.2}{\textbf{GAPN}} &
  \colorbox[HTML]{CBCEFB}{$0.12_{\pm 0.99}$} &
  \colorbox[HTML]{CBCEFB}{$0.12_{\pm 0.99}$} &
  \multicolumn{1}{c|}{\colorbox[HTML]{CBCEFB}{$0.12_{\pm 0.99}$}} &
 \colorbox[HTML]{CBCEFB}{$0.12_{\pm 0.99}$} &
  \colorbox[HTML]{CBCEFB}{$0.12_{\pm 0.99}$} &
  \multicolumn{1}{c|}{\colorbox[HTML]{CBCEFB}{$0.12_{\pm 0.99}$}} &
  \colorbox[HTML]{CBCEFB}{$0.12_{\pm 0.99}$} &
  \colorbox[HTML]{CBCEFB}{$0.12_{\pm 0.99}$} &
  \colorbox[HTML]{CBCEFB}{$0.12_{\pm 0.99}$} \\ \midrule
Ours vs. MoLPC &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} \\ \bottomrule
\end{tabular}%
}
\end{table*}

==> table/tmp.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}lccccccccc@{}}
\toprule
                                  & \multicolumn{3}{c}{GT dimer} & \multicolumn{3}{c}{AF-mm dimer} & \multicolumn{3}{c}{ESMFold dimer} \\ \cmidrule(l){2-10} 
\multirow{-2}{*}{\textbf{Methods}} &
  RMSD (\uparrow) &
  TM-Score (\uparrow) &
  \multicolumn{1}{c|}{DockQ (\uparrow)} &
  RMSD (\uparrow) &
  TM-Score (\uparrow) &
  \multicolumn{1}{c|}{DockQ (\uparrow)} &
  RMSD (\uparrow) &
  TM-Score (\uparrow) &
  DockQ (\uparrow) \\ \midrule
\multicolumn{1}{l|}{Multi-zerd}   &   &  & \multicolumn{1}{c|}{} &    &   & \multicolumn{1}{c|}{}  &           &           &           \\
\multicolumn{1}{l|}{RL-multizerd} &   &  & \multicolumn{1}{c|}{} &    &   & \multicolumn{1}{c|}{}  &           &           &           \\
\multicolumn{1}{l|}{AF-multimer}  &   &  & \multicolumn{1}{c|}{} &    &   & \multicolumn{1}{c|}{}  &           &           &           \\
\multicolumn{1}{l|}{ESMFold}      &   &  & \multicolumn{1}{c|}{} &    &   & \multicolumn{1}{c|}{}  &           &           &           \\
\multicolumn{1}{l|}{MoLPC}        &   &  & \multicolumn{1}{c|}{} &    &   & \multicolumn{1}{c|}{}  &           &           &           \\
\multicolumn{1}{l|}{\textbf{DiffDP}} &
  \cellcolor[HTML]{CBCEFB} &
  \cellcolor[HTML]{DAE8FC} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{CBCEFB}} &
  \cellcolor[HTML]{CBCEFB} &
  \cellcolor[HTML]{CBCEFB} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{CBCEFB}} &
  \cellcolor[HTML]{CBCEFB} &
  \cellcolor[HTML]{CBCEFB} &
  \cellcolor[HTML]{CBCEFB} \\ \midrule
Ours vs. MoLPC &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} \\ \bottomrule
\end{tabular}%
}
\end{table}
